Free Gap Estimates from the Exponential Mechanism, Sparse Vector, Noisy Max and Related Algorithms

Private selection algorithms, such as the Exponential Mechanism, Noisy Max and Sparse Vector, are used to select items (such as queries with large answers) from a set of candidates, while controlling privacy leakage in the underlying data. Such algorithms serve as building blocks for more complex differentially private algorithms. In this paper we show that these algorithms can release additional information related to the gaps between the selected items and the other candidates for free (i.e., at no additional privacy cost). This free gap information can improve the accuracy of certain follow-up counting queries by up to 66%. We obtain these results from a careful privacy analysis of these algorithms. Based on this analysis, we further propose novel hybrid algorithms that can dynamically save additional privacy budget.

==> proof_disc_laplace.tex <==
\printProofs[implement]

A discretized Laplace distribution whose support ranges over multiples of some base $\gamma$ has the following probability mass function:
%\begin{theorem}[Discrete Laplace \cite{universallyUtilityMaximizingPrivacyMechanisms}]\label{thm:disclaplace}
%Let $\vq$ be a vector-valued query, where each component of $\vq(D)$ is always a multiple of $\gamma$. Given a privacy loss budget $\epsilon$, consider the mechanism that returns $\vq(D)+H$, where $H$ is a vector of independent random samples from the DiscLaplace$(\Delta_{\vq}/\epsilon)$ distribution having probability mass function 
$f(k; \epsilon) = \frac{1-e^{-\gamma\epsilon}}{1+e^{-\gamma\epsilon}} e^{-\epsilon |k|}$ (for $k=0, \pm \gamma, \pm 2\gamma,\dots$). 
%This Discrete Laplace mechanism satisfies $\epsilon$-differential privacy. 
%\end{theorem}

%Let $\gamma$ be the base of the discrete laplace distribution. 
We will first consider the probability of a tie between two queries and then use the union bound over all pairs of queries.

Suppose $\eta_1$ and $\eta_2$ are two i.i.d zero mean discrete Laplace random variables with scale $1/\epsilon$ and base $\gamma$.
Without loss of generality, let $ q_1 - q_2 = m\gamma \geq 0$. Then the probability that $q_1+\eta_1 = q_2 + \eta_2$ is: 
\begingroup
\allowdisplaybreaks
\begin{align*}
    &\bbP(q_1+\eta_1 =q_2+ \eta_2) = \sum_{\ell\in\bbZ} \bbP(\eta_1 =  \gamma \ell)\bbP(\eta_2 =  (\ell+m)\gamma)\\%
    &=\frac{(1-e^{-\gamma\epsilon})^2}{(1+ e^{-\gamma\epsilon})^2} \sum_{\ell\in \bbZ} e^{-\epsilon\gamma\abs{\ell}} e^{-\epsilon\gamma\abs{\ell+m}}\\%
    &=\frac{(1-e^{-\gamma\epsilon})^2}{(1+ e^{-\gamma\epsilon})^2}  \Big( \sum_{\ell=-\infty}^{-m} e^{\epsilon\gamma \ell}e^{\epsilon\gamma(\ell+m)}\\%
     &\qquad + \sum_{\ell=-m+1}^{0} e^{\epsilon\gamma \ell}e^{-\epsilon\gamma(\ell+m)} + \sum_{\ell=1}^{\infty} e^{-\epsilon\gamma \ell}e^{-\epsilon\gamma(\ell+m)} \Big)\\
    %&=\lambda^2 \big( e^{\epsilon\gamma m}\sum_{n=-\infty}^{-m} e^{2\epsilon\gamma n}+ \sum_{n=-m+1}^{0} e^{-\epsilon\gamma m} + e^{-\epsilon\gamma m}\sum_{n=1}^{\infty} e^{-2\epsilon\gamma n} \big) \\
    %&=\lambda^2 \big( e^{\epsilon\gamma m} \frac{e^{-2\epsilon\gamma m}}{1 - e^{-2\epsilon\gamma}} + m e^{-\epsilon\gamma m} + e^{-\epsilon\gamma m} \frac{e^{-2\epsilon\gamma}}{1 - e^{-2\epsilon\gamma}} \big)\\
    &=\frac{(1-e^{-\gamma\epsilon})^2}{(1+ e^{-\gamma\epsilon})^2} e^{-\epsilon\gamma m} \big(\frac{1}{1-e^{-2\epsilon\gamma}} + m + \frac{e^{-2\epsilon\gamma}}{1-e^{-2\epsilon\gamma}}\big)\\
    %&=\lambda^2 e^{-\epsilon\gamma m} (\frac{1+e^{-2\epsilon\gamma}}{1 - e^{-2\epsilon\gamma}} + m)\\
    &= \frac{(1-e^{-\gamma\epsilon})^2}{(1+ e^{-\gamma\epsilon})^2} e^{-\epsilon\gamma m} (\frac{1+e^{-2\epsilon\gamma}}{1 - e^{-2\epsilon\gamma}} + m)\\
    &\leq  \left(1-e^{-\gamma\epsilon}\right)^2e^{-\epsilon\gamma m}\left(\frac{1}{1-e^{-2\epsilon\gamma}}+m\right)\\
    &\leq  \left(1-e^{-\gamma\epsilon}\right)^2e^{-\epsilon\gamma m}\left(\frac{1}{1-e^{-\epsilon\gamma}}+m\right)\\
    &\leq (1-e^{-\gamma\epsilon}) +  \left(1-e^{-\gamma\epsilon}\right)^2e^{-\epsilon\gamma m}m\\
    &\leq \gamma\epsilon +  \left(1-e^{-\gamma\epsilon}\right)^2e^{-\epsilon\gamma m}m\quad\text{(since $1-e^{-x}\leq x$ for $x\geq -1$)}\\
    &\leq \gamma\epsilon + (\gamma\epsilon)^2me^{-\epsilon\gamma m} =\gamma\epsilon (1 + \gamma\epsilon m e^{-\gamma\epsilon m})\\
    &\leq \gamma\epsilon(1+e^{-1}) \quad\text{(since $xe^{-x}$ is maximized at $x=1$)}
\end{align*}
\endgroup
Since there are $n$ queries, we can conservatively estimate the probability of a tie as the probability that any pair of $n$ items has a tie. Using the union bound, we get the probability of a tie is at most $n^2 \gamma\epsilon$. In floating point, we expect a Laplace distribution to be implemented using a Discrete Laplace with $\gamma$ being close to machine epsilon, which for double-precision floating point numbers is around $2^{-52}$.


==> sec_new.tex <==
\clearpage
\subsection{\gaptopk with Exponential Noise}


% \begin{algorithm}[ht]
% \SetKwProg{Fn}{function}{\string:}{}
% \SetKwFunction{Test}{\funcgaptopk}
% \SetKwInOut{Input}{input}
% \DontPrintSemicolon
% \Input{$\vq$: a list of $n$ queries of global sensitivity 1\\
% $D$: database, $k$: \# of indexes, $\epsilon$: privacy budget}
% \Fn{\Test{$\vq$, $D$, $k$, $\epsilon$}}{
% \ForEach{$\mathtt{i} \in \set{1, \cdots, n}$}{
% $\eta_i \gets \fbox{$\Exp(2k/\epsilon)$}$\;
% $\widetilde{q}_i \gets q_i(D)+\eta_i$\;
% }
% $(j_1,\ldots, j_{k+1}) \gets \arg\max_{k+1}(\widetilde{q}_1,\ldots, \widetilde{q}_n)$\;
% \ForEach{$\mathtt{i} \in \set{1, \cdots, k }$}{
% \fbox{$g_{i} \gets \widetilde{q}_{j_i} - \widetilde{q}_{j_{i+1}}$ ~~~~~~\tcp{$i^{th}$ gap}}\label{line:gapdef}
% }
% \Return $((j_1\fbox{, $g_1$}),\ldots, (j_k \fbox{, $g_k$}))$\label{line:gapreturn} \tcp{$k$ queries}
% }
% \caption{\gaptopk}
% \label{alg:gaptopk}
% \end{algorithm}

% Recall the alignment for \gaptopk:
% \begin{equation}
% \eta_i' =\begin{cases}
% \eta_i &i\in\ioc\\
% \eta_i + q_i-q'_i+\max\limits_{l\in\ioc}(q_l'+\eta_l)- \max\limits_{l\in\ioc}(q_l+\eta_l)  &i\in\io
% \end{cases}    
% \end{equation}
% Let 
% \[s = \argmax\limits_{l\in \ioc}(q_l + \eta_l), t = \argmax\limits_{l\in \ioc}(q'_l + \eta_l)\]

% We have 
% \begin{equation}
% \eta_i' - \eta_i =\begin{cases}
% 0 &i\in\ioc\\
%  q_i-q'_i+(q'_{t}+\eta_{t})- (q_{s}+\eta_{s})  &i\in\io
% \end{cases}    
% \end{equation}

% Let 
% \begin{align*}
%     i_{*} &= \argmin_{i\in\io}\set{q_i-q'_i+(q'_{t}+\eta_{t})- (q_{s}+\eta_{s})} \\
%     \Delta\eta_{\min} &=  \min_{i\in\io}\set{q_i-q'_i+(q'_{t}+\eta_{t})- (q_{s}+\eta_{s})} \\
%     & = q_{i_{*}}-q'_{i_{*}}+(q'_{t}+\eta_{t})- (q_{s}+\eta_{s})
% \end{align*}

% When $\Delta\eta_{\min} < 0$,  the alignment is 
% \begin{equation}
% \eta_i'' =\begin{cases}
% \eta_i' &i\in\ioc\setminus\set{t}\\
% \eta_i' - \Delta\eta_{\min}  &i\in\io\cup\set{t}
% \end{cases}\\    
% =\begin{cases}
% \eta_i &i\in\ioc\setminus\set{t}\\
% \eta_i + q_i-q'_i - (q_{i_*} -q'_{i_*})  &i\in\io\cup\set{t}
% \end{cases}   
% \end{equation}


% To see why this works, 
% \begin{align*}
%     \abs{\eta''_i -\eta_i} &= q_i - q'_i - (q_{i_*} - q'_{i_*}) \leq 2 &i\in \io\\
%     \abs{\eta''_t -\eta_t} &= q_{i_{*}}-q'_{i_{*}}+(q'_{t}+\eta_{t})- (q_{s}+\eta_{s}) \leq 2\\
%     \abs{\eta''_i -\eta_i} &= 0 &i\in\ioc\setminus\set{t}\\
% \end{align*}
% Moreover, $\abs{\eta''_{i_*} -\eta_{i_*}} = 0$. Thus
% \begin{align*}
% \cost&(\alio) =\sum_{i=1}^\infty\abs{\eta_i''-\eta_i} \frac{\epsilon}{2k}\\
% \leq&\frac{\epsilon}{2k}\sum_{i\in\cI_\omega\cup\set{t}\setminus\set{i_*}}2 =\frac{\epsilon}{2k}\cdot 2\cdot k = \epsilon.
% \end{align*}



% \subsection{Noisy Top-k with Threshold}
% We consider a variant of Noisy Max/Top-k that takes one additional parameter $T$ as a threshold and release the identities of up to $k$ queries that are approximately maximum and above the threshold $T$.

% \begin{algorithm}[ht]
% \SetKwProg{Fn}{function}{\string:}{}
% \SetKwFunction{Test}{\funcgapmax}
% \SetKwInOut{Input}{input}
% \DontPrintSemicolon
% \Input{$\vq$: a list of $n$ queries of global sensitivity 1, $T$: threshold
% $D$: database, $k$: \# of indexes, $\epsilon$: privacy budget}
% \Fn{\Test{$\vq$, $T$, $D$, $k$, $\epsilon$}}{
% $bq = T + \lap(2/\epsilon)$, $sbq = -\infty$, $max=0$\;
% \ForEach{$\mathtt{i} \in \set{1, \cdots, n}$}{
% $\eta_i \gets \lap(2/\epsilon)$\;
% $\widetilde{q}_i \gets q_i(D)+\eta_i$\;
% \uIf{$\widetilde{q}_i > bq$}{
% $sbq = bq$ \;
% $bq = \widetilde{q}_i$ \;
% $max = i$
% }
% \ElseIf{$\widetilde{q}_i > sbq$}{
% $sbq = \widetilde{q}_i$
% }
% }
% %$(j_1,\ldots, j_{k+1}) \gets \arg\max_{k+1}(\widetilde{q}_1,\ldots, \widetilde{q}_n)$\;
% %\ForEach{$\mathtt{i} \in \set{1, \cdots, k }$}{
% %\fbox{$g_{i} \gets \widetilde{q}_{j_i} - \widetilde{q}_{j_{i+1}}$ ~~~~~~\tcp{$i^{th}$ gap}}\label{line:gapdef}
% %}
% %\Return $((j_1\fbox{, $g_1$}),\ldots, (j_k \fbox{, $g_k$}))$\label{line:gapreturn} \tcp{$k$ queries}
% \Return $max, bq-sbq$
% }
% \caption{NoisyMax-w-Gap-n-Threshold}
% \label{alg:gaptopkwitht}
% \end{algorithm}








\todo{New stuff to be added:
\begin{itemize}
    \item \checkmark Sparse with exponential noise 
    \item \checkmark Noisy-top-k with exponential noise
    \item \checkmark Sparse Vector with Gap with (one-sided) geometric noise
    \item (?) Noisy Max/Top-k with Gap with geometric noise
    \item \checkmark Exponential mechanism with gap from logistic distribution
\end{itemize}

}

\textbf{Scratch Paper}







\noindent\rule[0.5ex]{\linewidth}{1pt}
Question: 

let $f(x)=\text{Gumble}(x;\mu,\beta)= \exp(-\frac{(x-\mu)}{\beta} - e^{-\frac{(x-\mu)}{\beta}})$
\begin{align*}
    \ln \frac{f(x)}{f(y)} &= (-\frac{(x-\mu)}{\beta} - e^{-\frac{(x-\mu)}{\beta}}) - (-\frac{(y-\mu)}{\beta} - e^{-\frac{(y-\mu)}{\beta}})\\
    &=\frac{y-x}{\beta} + e^{-\frac{(y-\mu)}{\beta}} - e^{-\frac{(x-\mu)}{\beta}}\\
    &= \cdots \\
    &?= O(\abs{y-x})
\end{align*}

\subsection{If Program}
\begin{lemma}
Let $e$ be a random Boolean expression. Let $p(D) = \prob{e = \true \mid D}$, i.e., the probability of $e$ when the input is $D$.
If 
\begin{enumerate}
    \item $\max_{D\sim D'}(\ln\frac{p(D')}{p(D)}, \ln\frac{1-p(D')}{1-p(D)}) \leq \epsilon_1$, and
    \item $c_1, c_2$ are $\epsilon_2$-DP,
\end{enumerate} then
$\ifcmd{e}{(c_1)}{(c_2)}$ is $(\epsilon_1 + \epsilon_2)$-DP.
\end{lemma}



\subsection{While Program}
\begin{lemma}
Let $e$ be a random Boolean expression and $c$ an arbitrary program. Let $p_n(D)$ be the probability of $e$ after executing $c$ $n$ times with input $D$.
If 
\begin{enumerate}
    \item $\forall k> 0, \forall D\sim D'$, $\sum_{i=0}^{k-1}\ln\frac{p_i(D')}{p_i(D)} + \ln\frac{1-p_k(D')}{1-p_k(D)} \leq \epsilon_1$, and
    \item $c$ is $\epsilon_2$-DP,
\end{enumerate} then
$\whilecmd{e}{(c)}$ is $(\epsilon_1 + \epsilon_2)$-DP.
\end{lemma}



\textbf{End Scratch Paper}

\noindent\rule[0.5ex]{\linewidth}{1pt}


